Low latency via redundancy

Low latency is critical for interactive networked applications. But while we know how to scale systems to increase capacity, reducing latency --- especially the tail of the latency distribution --- can be much more difficult. In this paper, we argue that the use of redundancy is an effective way to convert extra capacity into reduced latency. By initiating redundant operations across diverse resources and using the first result which completes, redundancy improves a system's latency even under exceptional conditions. We study the tradeoff with added system utilization, characterizing the situations in which replicating all tasks reduces mean latency. We then demonstrate empirically that replicating all operations can result in significant mean and tail latency reduction in real-world systems including DNS queries, database servers, and packet forwarding within networks.

==> cost-benefit.tex <==
\subsection{Individual view: cost-benefit analysis}
\label{sec:cost-benefit}

The model and experiments of the previous section indicated that in a range of scenarios, latency is best optimized in a fixed set of system resources through replication.  However, some systems are better modeled as having \emph{elastic} resources:  individual participants can choose whether to replicate an operation, but this incurs monetary cost.  In this section, our goal is to estimate in what scenarios replication is cost-effective.  This, of course, depends strongly upon the specific system's value of latency and cost of resources.  Here we estimate costs and benefits within a limited but useful class of systems: a wide-area client-server application (such as web browsing, DNS queries, etc.) involving a client using consumer-level connectivity and a service provider in the cloud.  This serves as a baseline model which may be refined or extended for other systems; we will compare to this baseline when we discuss several applications later.

We can estimate when replication is useful for an individual operation via the value of time and the cost of increased utilization. As a convenience, we will measure increased utilization in units of bandwidth.  For replication to be beneficial, we need $\ell v \geq c$, where $\ell$ is the average latency savings in milliseconds for each KB of added traffic, $v$ is the dollar value of one millisecond of latency reduction, and $c$ is the cost of added traffic per KB.  Our goal is to find a threshold value of $\ell$ when replication becomes beneficial.  For this, we need estimates of $c$ and $v$. These are very different on the client and server sides.

\begin{table*}
\small
\begin{center}
\begin{tabular}{l|r@{\extracolsep{0pt}.}l|r@{\extracolsep{0pt}.}lr@{\extracolsep{0pt}.}l}
\hline 
Service plan & \multicolumn{2}{c|}{Cost $b$} & \multicolumn{4}{c}{Break-even benefit $\ell$ (msec/KB), assuming...}\\
 & \multicolumn{2}{c|}{(\$/GB)} & \multicolumn{2}{c}{server-side $\$0.76$/hr value} & \multicolumn{2}{c}{client-side $\$23.73$/hr value}\\
\hline 
\hline 
\emph{Server-side plans} & \multicolumn{2}{c|}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{}\\
~~~Amazon web services: ``Common Customer'' web app & 3&68 & ~~~~~~~~~~~~16&62 & ~~~~~~~~~~~~&53\tabularnewline
~~~Amazon Route 53 (DNS) assuming 0.5KB/query & 1&05 & 4&74 & &15\\
~~~NearlyFreeSpeech.net: small-volume web hosting & 1&00 & 4&51 & &14\\
~~~Amazon CloudFront: U.S., 1 GB/mo, 1 KB/object & &91 & 4&11 & &13\\
~~~NearlyFreeSpeech.net: large-volume web hosting & &20 & &90 & &029\\
~~~Amazon CloudFront: U.S., 1 GB/mo, 10 KB/object & &20 & &90 & &029\\
~~~Amazon EC2 and Microsoft Azure: bandwidth only & &12 & &54 & &017\\
~~~MaxCDN: based on ``starter'' plan overage fee & &07 & &32 & &010\\
~~~DreamHost: cloud storage, object delivery & &07 & &32 & &010\\
 & \multicolumn{2}{c|}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{}\\
\emph{Client-side plans} & \multicolumn{2}{c|}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{}\\
~~~AT\&T, low volume cell plan, based on overage fees & ~61&40 & 277&37 & 8&88\\
~~~AT\&T, high volume cell plan, based on overage fees & 10&00 & 45&17 & 1&45\\
~~~O$_{2}$ mobile broadband, based on 1GB$\to$2GB increment & 5&10 & 23&04 & &74\\
~~~AT\&T DSL & &20 & &90 & &029\\
\hline 
\end{tabular}
\end{center}
\caption{Estimates of the cost of added utilization (in GB of data transfer), and resulting threshold benefit $\ell$ (in milliseconds saved per KB of added utilization) at which replication becomes cost-effective. Based on providers' publicly advertised prices as of December 2012, excluding taxes and fees.}
\label{table:cost-benefit}
\end{table*}


\parheading{Cost estimates.}  To estimate the cost $c$, we use a range of advertised rates for cloud services which implement usage-based pricing, listed in the second column of Table~\ref{table:cost-benefit}.  Note that while we measure utilization in units of data transfer volume, listed costs include services besides bandwidth.  The most expansive (and expensive) of these is the first line, based on an Amazon Web Services sample customer profile of a web application.\footnote{\url{http://calculator.s3.amazonaws.com/calc5.html#key=a-simple-3-tier-web-app}}  The profile models a 3-tier auto-scalable web application, with a load balancer, two web servers, two app servers, a high-availability database server, 30 GB of storage, and other services, which utilizes $120$ GB/month of data transfer out of EC2 and $300$ GB/month out of CloudFront.  The resulting amortized cost of \$$3.68$ effectively models the cost (per transferred GB) of an average operation in this system, including the cost of all utilized services.\footnote{This is likely pessimistic since it includes, for example, the cost of increased storage which would not scale linearly with an increase in service operations.}  The other services listed in the table model the cost of more limited operations, such as DNS or bandwidth alone.

On the client side, we limit this investigation to clients in which the dominant cost of incrementally added utilization is due to network bandwidth.  Table~\ref{table:cost-benefit} lists costs based on several types of connectivity. For these calculations, we assume a user who has paid for basic connectivity already, and calculate the cost of bandwidth from overage charges. Client-side bandwidth costs can be substantially higher than server-side total costs in extreme (cellular) cases but are comparable or cheaper with DSL connectivity.

Of course, there are scenarios which the above range of application costs does not model. For example, a cellular client whose battery is nearly empty may value energy more than bandwidth.  But in a large class of situations, bandwidth is the most constrained resource on the client.


%The value of time $v$ may be highly application-specific; the target might be the tail latency, the mean, or a more complex objective.

\parheading{Value estimates.} The value of time $v$ is more difficult to calculate, at both the client and server.

For the server, direct value may come from obtaining revenue (ads, sales).  We consider the case of Google.  A study by Google indicated that users experiencing an artifical $400$ ms added delay on each search performed $0.74$\% fewer searches after 4-6 weeks~\cite{brutlag09}.  Google's revenue per search has been estimated\footnote{Based on forecasts at \url{http://www.trefis.com}.} at \$$0.017$; therefore, we can estimate a savings of $400$ milliseconds on a single search generates, on average, an additional $\$0.0168\cdot0.0074$ in revenue, or \$$1.12$ per hour of reduced latency.  As another estimate, a $500$ millisecond delay in the Bing search engine reduced revenue per user by $1.2$\%, or $4.3$\% with a $2$-second delay~\cite{souders09velocity}. Using the latter (smaller) figure, combined with an estimated\footnote{\url{http://www.trefis.com/company?hm=MSFT.trefis&driver=idMSFT.0817#}} revenue per search of $\$0.00976$, we have a \$$0.76$ per hour value. We use the more pessimistic Bing value of \$$0.76$/hr in our calculations.

On the client side, value may be obtained from a better or faster human experience.  Among all the components of our analysis, this value is the hardest to estimate: it may be highly application-specific, and may depend on mean or tail latency in ways best quantified by a human user study of quality of experience.  But as a first approximation, we assume the value of time is simply the US average earnings of \$23.73 per hour in December 2012~\cite{avgHourlyWage}, which implies $v \approx 6.59 \cdot 10^{-6} ~\$/\textrm{ms}$.

\parheading{Finding the threshold.}  We can now use our cost and value estimates to solve $\ell \geq c / v$ to obtain the break-even point, in terms of the necessary latency savings per kilobyte of additional traffic.

Table~\ref{table:cost-benefit} shows the break-even values of $\ell$ for each scenario. The values are divided into four quadrants. The upper-left quadrant shows $\ell$ from the perspective of a server making a selfish decision.  For example, the table indicates that a server replicating DNS traffic would obtain greater return in ad revenue than the cost of increased utilization, as long as replication saves more than $4.74$ milliseconds per KB of added traffic.

Some servers may directly value the client's quality of service.  The upper-right quadrant of the table shows the necessary break-even benefit above which the client's value outweighs the server's costs.  Similarly, the lower-right quadrant shows the break-even benefit for a client choosing to replicate its traffic.

The lower-left quadrant indicates the threshold beyond which the \emph{server's benefit} outweighs the \emph{client's costs}.  This is unrealistic: a client would not typically value the server's ad revenue yet ignore its own benefit.

In general, the break-even threshold varies by several orders of magnitude depending on the assumed costs and benefits.  But interestingly, excluding the latter unrealistic scenario, both the server's and the client's most pessimistic break-even benefit occurs in a similar range of $8$-$16$ ms/KB; the client's higher costs are roughly balanced by its greater benefit.  This analysis suggests that \emph{replication may be cost-effective even in the most conservative cases as long as we can save more than $\approx$ 8-16 milliseconds (in the mean or tail, depending on the goal) for each kilobyte of added traffic.}

The above analysis, of course, depends on the unknown accuracy of several estimates. But as we will see next, real-world applications can obtain benefit \emph{at least an order of magnitude} greater than the $8$-$16$ ms/KB threshold.

% First, the upper-left quadrant, corresponding to a selfish server, does not depend on our (relatively uncertain) estimate of the client's value of time.  Second, 

% ATT DSL overage charge: $10 per 50 GB
%http://www.att.com/Common/indc/popup/internet_terms_conditions.htm

% Cell charge refs
% Overage, plan 1: $14.99 per 250 MB
% Overage, plan 2: $10 per 1 GB
% Ref: http://www.att.com/shop/wireless/data-plans.html

% ATT caps DSL at 150 GB
% http://www.cnn.com/2011/TECH/web/03/15/att.broadband.allowance.wired/index.html
% Actually ATT now says 250 GB on some accounts...
% http://www.att.com/gen/general?pid=7689

% ATT DSL is $20/mo
% http://www.att.com/dsl/shop/plansShared.jsp

% US average hourly earnings Dec 2012 for all employees on private nonfarm payrolls: \$23.73
% http://www.bls.gov/eag/eag.us.htm/


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 

